Macroscopic behavior of Lipschitz random surfaces

The motivation for this article is to derive strict convexity of the surface tension for Lipschitz random surfaces, that is, for models of random Lipschitz functions from $\mathbb Z^d$ to $\mathbb Z$ or $\mathbb R$. An essential innovation is that random surface models with long- and infinite-range interactions are included in the analysis. More specifically, we cover at least: uniformly random graph homomorphisms from $\mathbb Z^d$ to a $k$-regular tree for any $k\geq 2$ and Lipschitz potentials which satisfy the FKG lattice condition. The latter includes perturbations of dimer- and six-vertex models and of Lipschitz simply attractive potentials introduced by Sheffield. The main result is that we prove strict convexity of the surface tension -- which implies uniqueness for the limiting macroscopic profile -- if the model of interest is monotone in the boundary conditions. This solves a conjecture of Menz and Tassy, and answers a question posed by Sheffield. Auxiliary to this, we prove several results which may be of independent interest, and which do not rely on the model being monotone. This includes existence and topological properties of the specific free energy, as well as a characterization of its minimizers. We also prove a general large deviations principle which describes both the macroscopic profile and the local statistics of the height functions. This work is inspired by, but independent of, Random Surfaces by Sheffield.

==> figures/truncation/data.tex <==
\draw(0,-0.0)--(200,-40.0);
\draw(0,0.0)--(20,-4.0)--(100,60.0)--(180,-36.0)--(200,-40.0);
\draw(0,12.0)--(20,8.0)--(100,72.0)--(180,-24.0)--(200,-28.0);
\draw(0,24.0)--(20,20.0)--(100,84.0)--(180,-12.0)--(200,-16.0);
\draw(0,-0.0)--(20,-4.0)--(100,-100.0)--(180,-36.0)--(200,-40.0);
\draw(0,-12.0)--(20,-16.0)--(100,-112.0)--(180,-48.0)--(200,-52.0);
\draw(0,-24.0)--(20,-28.0)--(100,-124.0)--(180,-60.0)--(200,-64.0);
\draw(0,0.0)--(1,5.3012295074708735)--(2,6.961260683447953)--(3,6.661200318076056)--(4,-0.8736913672924318)--(5,-4.225192025995522)--(6,-0.6752865723778346)--(7,-4.804844165215168)--(8,-11.382074694779803)--(9,-15.323030889443242)--(10,-18.8921303835474)--(11,-16.252925463491902)--(12,-23.298074322966816)--(13,-26.222504349659076)--(14,-30.275796866798363)--(15,-26.578635505060166)--(16,-23.402591114645)--(17,-28.796803562466067)--(18,-28.331034948516848)--(19,-28.12932202129731)--(20,-35.198006522956156)--(21,-36.62359426073721)--(22,-30.47815784919469)--(23,-34.55602799536713)--(24,-39.9730310680455)--(25,-35.907991229349854)--(26,-41.64089388093422)--(27,-43.60902154475391)--(28,-36.31017235445313)--(29,-30.605765574122596)--(30,-34.60877461391778)--(31,-28.539307746499663)--(32,-33.98007745613776)--(33,-28.16638058426398)--(34,-35.686259414318776)--(35,-29.130344316551223)--(36,-32.52481468523513)--(37,-37.82149626991834)--(38,-33.733863002400064)--(39,-36.3783907247685)--(40,-32.077107249702834)--(41,-27.472575270636252)--(42,-30.974460084135373)--(43,-37.820907251454464)--(44,-34.169690273585395)--(45,-35.540260020824334)--(46,-37.10860761748474)--(47,-42.98957982398231)--(48,-43.92956903685247)--(49,-37.8301666383021)--(50,-37.124744269771)--(51,-42.068923055506644)--(52,-41.31554196379819)--(53,-43.53141216679537)--(54,-40.81775686118024)--(55,-44.221745390487186)--(56,-50.951255182603404)--(57,-57.40317428155389)--(58,-49.59172634578511)--(59,-49.06038091629415)--(60,-42.298956694572865)--(61,-36.09372615037469)--(62,-28.61499689672624)--(63,-32.53456555232996)--(64,-27.308245636686493)--(65,-34.65050491725552)--(66,-30.849494109166976)--(67,-35.60581505540362)--(68,-39.11855340918012)--(69,-45.53660416910927)--(70,-49.77953806245395)--(71,-53.29538675804117)--(72,-56.1351292497961)--(73,-50.594974837401324)--(74,-53.03290400622324)--(75,-52.6000815734782)--(76,-56.189859518755384)--(77,-50.33903888244133)--(78,-48.99535804307217)--(79,-43.80494898541555)--(80,-46.62146775447714)--(81,-47.40949938001217)--(82,-40.83799525423281)--(83,-39.03458106219348)--(84,-36.75165953402373)--(85,-32.78971111399299)--(86,-30.987110585756515)--(87,-24.06454510946141)--(88,-24.040887963117896)--(89,-25.814828249391304)--(90,-19.421349118681885)--(91,-19.56899411695857)--(92,-22.474718173702136)--(93,-15.938579338612854)--(94,-17.72795628748892)--(95,-16.80687680004351)--(96,-15.120980389207803)--(97,-10.44223514985535)--(98,-4.444882810609173)--(99,0.44377579984027005)--(100,0.35496255098636276)--(101,1.0767271293386758)--(102,-3.3363718920642924)--(103,-1.602232347812512)--(104,2.3667978596305472)--(105,6.85430633927545)--(106,6.887869373573688)--(107,8.211735955349939)--(108,6.726462662519838)--(109,-0.2102666240940323)--(110,-3.083495157299044)--(111,-1.6951118662161857)--(112,-2.899179422511759)--(113,3.135737585729216)--(114,-4.28226532088221)--(115,-11.033986073515596)--(116,-4.146466607540233)--(117,-6.551282420149123)--(118,-11.552357571236536)--(119,-11.642250627744618)--(120,-11.916682961400655)--(121,-14.255048540820205)--(122,-20.69866867740767)--(123,-24.068072079364786)--(124,-22.10513027198744)--(125,-29.85092447410317)--(126,-32.81105050555818)--(127,-36.669076244841854)--(128,-38.68777793504141)--(129,-35.33679118613895)--(130,-42.20889412695256)--(131,-40.415158985517486)--(132,-35.245345710017546)--(133,-28.16869559833743)--(134,-20.817635958992945)--(135,-18.548781923266226)--(136,-12.911049108001952)--(137,-20.471386944232265)--(138,-17.248028903364357)--(139,-23.140780244591447)--(140,-25.27347829101077)--(141,-19.706032586039846)--(142,-18.626532980304674)--(143,-17.313160921571196)--(144,-17.26433861159451)--(145,-16.053646143277682)--(146,-21.416441308604067)--(147,-19.46766266626096)--(148,-18.915147036661303)--(149,-20.77627443039549)--(150,-21.471274509503708)--(151,-19.04139312935944)--(152,-26.557489263926968)--(153,-22.113010540283693)--(154,-22.22218043698998)--(155,-15.440315001540917)--(156,-14.088804576032064)--(157,-18.806757112741103)--(158,-11.366927734149185)--(159,-13.553520078849884)--(160,-13.237350285809788)--(161,-15.988029240730308)--(162,-8.163040809607729)--(163,-13.791645770639553)--(164,-21.907308463387338)--(165,-16.47291056694808)--(166,-14.587963144181966)--(167,-8.058312661348062)--(168,-0.8954942836333828)--(169,-1.2721930869469187)--(170,5.966470705709242)--(171,2.313045743030367)--(172,9.381180183938554)--(173,7.636498315517409)--(174,11.082059478371296)--(175,8.026635396244957)--(176,15.798055032167598)--(177,14.400223778222554)--(178,7.7667741380077855)--(179,0.9319224684183176)--(180,4.215600309082275)--(181,1.4690809196942105)--(182,-4.132306431623649)--(183,-4.902286028309119)--(184,-5.219563784795339)--(185,-3.7925737686655197)--(186,-0.243307564562512)--(187,-4.048647962053458)--(188,-5.157147251193392)--(189,-0.4036927064694211)--(190,-1.8706418844847406)--(191,-5.192934855606662)--(192,0.06482332612696595)--(193,-6.538328529239919)--(194,-12.737667963746931)--(195,-13.185173587585998)--(196,-9.047880749495741)--(197,-5.587754402208647)--(198,-2.910009484736488)--(199,-4.309803545910075)--(200,0.0);
\draw(0,0.0)--(1,5.3012295074708735)--(2,6.961260683447953)--(3,6.661200318076056)--(4,-0.8736913672924318)--(5,-4.225192025995522)--(6,-0.6752865723778346)--(7,-4.804844165215168)--(8,-11.382074694779803)--(9,-15.323030889443242)--(10,-18.8921303835474)--(11,-16.252925463491902)--(12,-23.298074322966816)--(13,-26.222504349659076)--(14,-30.275796866798363)--(15,-26.578635505060166)--(16,-23.402591114645)--(17,-28.796803562466067)--(18,-28.331034948516848)--(19,-28.12932202129731)--(20,-35.198006522956156)--(21,-36.62359426073721)--(22,-30.47815784919469)--(23,-34.55602799536713)--(24,-39.9730310680455)--(25,-35.907991229349854)--(26,-41.64089388093422)--(27,-43.60902154475391)--(28,-36.31017235445313)--(29,-30.605765574122596)--(30,-34.60877461391778)--(31,-28.539307746499663)--(32,-33.98007745613776)--(33,-28.16638058426398)--(34,-35.686259414318776)--(35,-29.130344316551223)--(36,-32.52481468523513)--(37,-37.82149626991834)--(38,-33.733863002400064)--(39,-36.3783907247685)--(40,-32.077107249702834)--(41,-27.472575270636252)--(42,-30.974460084135373)--(43,-37.820907251454464)--(44,-34.169690273585395)--(45,-35.540260020824334)--(46,-37.10860761748474)--(47,-42.98957982398231)--(48,-43.92956903685247)--(49,-37.8301666383021)--(50,-37.124744269771)--(51,-42.068923055506644)--(52,-41.31554196379819)--(53,-43.53141216679537)--(54,-40.81775686118024)--(55,-44.221745390487186)--(56,-50.951255182603404)--(57,-57.40317428155389)--(58,-49.59172634578511)--(59,-49.06038091629415)--(60,-42.298956694572865)--(61,-36.09372615037469)--(62,-28.61499689672624)--(63,-32.53456555232996)--(64,-27.308245636686493)--(65,-34.65050491725552)--(66,-30.849494109166976)--(67,-35.60581505540362)--(68,-39.11855340918012)--(69,-45.53660416910927)--(70,-49.77953806245395)--(71,-53.29538675804117)--(72,-56.1351292497961)--(73,-50.594974837401324)--(74,-53.03290400622324)--(75,-52.6000815734782)--(76,-56.189859518755384)--(77,-50.33903888244133)--(78,-48.99535804307217)--(79,-43.80494898541555)--(80,-46.62146775447714)--(81,-47.40949938001217)--(82,-40.83799525423281)--(83,-39.03458106219348)--(84,-36.75165953402373)--(85,-32.78971111399299)--(86,-30.987110585756515)--(87,-24.06454510946141)--(88,-24.040887963117896)--(89,-25.814828249391304)--(90,-19.421349118681885)--(91,-19.56899411695857)--(92,-22.474718173702136)--(93,-15.938579338612854)--(94,-17.72795628748892)--(95,-16.80687680004351)--(96,-15.120980389207803)--(97,-10.44223514985535)--(98,-4.444882810609173)--(99,0.44377579984027005)--(100,0.35496255098636276)--(101,1.0767271293386758)--(102,-3.3363718920642924)--(103,-1.602232347812512)--(104,2.3667978596305472)--(105,6.85430633927545)--(106,6.887869373573688)--(107,8.211735955349939)--(108,6.726462662519838)--(109,-0.2102666240940323)--(110,-3.083495157299044)--(111,-1.6951118662161857)--(112,-2.899179422511759)--(113,3.135737585729216)--(114,-4.28226532088221)--(115,-11.033986073515596)--(116,-4.146466607540233)--(117,-6.551282420149123)--(118,-11.552357571236536)--(119,-11.642250627744618)--(120,-11.916682961400655)--(121,-14.255048540820205)--(122,-20.69866867740767)--(123,-24.068072079364786)--(124,-22.10513027198744)--(125,-29.85092447410317)--(126,-32.81105050555818)--(127,-36.669076244841854)--(128,-38.68777793504141)--(129,-35.33679118613895)--(130,-42.20889412695256)--(131,-40.415158985517486)--(132,-35.245345710017546)--(133,-28.16869559833743)--(134,-20.817635958992945)--(135,-18.548781923266226)--(136,-12.911049108001952)--(137,-20.471386944232265)--(138,-17.248028903364357)--(139,-23.140780244591447)--(140,-25.27347829101077)--(141,-19.706032586039846)--(142,-18.626532980304674)--(143,-17.313160921571196)--(144,-17.26433861159451)--(145,-16.053646143277682)--(146,-21.416441308604067)--(147,-19.46766266626096)--(148,-18.915147036661303)--(149,-20.77627443039549)--(150,-21.471274509503708)--(151,-19.04139312935944)--(152,-26.557489263926968)--(153,-22.113010540283693)--(154,-22.22218043698998)--(155,-15.440315001540917)--(156,-14.088804576032064)--(157,-18.806757112741103)--(158,-11.366927734149185)--(159,-13.553520078849884)--(160,-13.237350285809788)--(161,-15.988029240730308)--(162,-8.163040809607729)--(163,-13.791645770639553)--(164,-21.907308463387338)--(165,-16.47291056694808)--(166,-14.587963144181966)--(167,-8.058312661348062)--(168,-0.8954942836333828)--(169,-1.2721930869469187)--(170,-16.525585193233887)--(171,-14.17401311090319)--(172,-23.142018654253473)--(173,-17.698727670787573)--(174,-21.485399902562612)--(175,-26.900027778138142)--(176,-19.5757650726945)--(177,-29.57130629899078)--(178,-25.95419339251414)--(179,-30.41272223330651)--(180,-24.762700296397924)--(181,-24.54391848554859)--(182,-25.863313449736065)--(183,-28.182858980523836)--(184,-31.643150641242407)--(185,-32.216704844894)--(186,-26.920366678444594)--(187,-27.273210457752413)--(188,-36.862777847259736)--(189,-26.409458862421175)--(190,-30.674992799923757)--(191,-26.699022753917998)--(192,-32.10794907590446)--(193,-33.43206807249254)--(194,-38.03415492607712)--(195,-35.55016373674483)--(196,-31.84849648604176)--(197,-29.83000646057277)--(198,-38.041709436032484)--(199,-29.687095961210716)--(200,-36.40639258510084);
\draw(0,0.0)--(1,5.3012295074708735)--(2,6.961260683447953)--(3,6.661200318076056)--(4,-0.8736913672924318)--(5,-4.225192025995522)--(6,-0.6752865723778346)--(7,-4.804844165215168)--(8,-11.382074694779803)--(9,-15.323030889443242)--(10,-18.8921303835474)--(11,-16.252925463491902)--(12,-23.298074322966816)--(13,-26.222504349659076)--(14,-4.702007941022742)--(15,-26.578635505060166)--(16,-23.402591114645)--(17,-15.005497204858944)--(18,-8.335852633615719)--(19,-11.909722571725101)--(20,-10.354532723354126)--(21,-6.040889496730662)--(22,-7.792086830399798)--(23,-12.80272945906366)--(24,-13.204811350196728)--(25,-18.544516205832)--(26,-16.900732490133663)--(27,-23.945797335412536)--(28,-36.31017235445313)--(29,-30.605765574122596)--(30,-34.60877461391778)--(31,-28.539307746499663)--(32,-33.98007745613776)--(33,-28.16638058426398)--(34,-35.686259414318776)--(35,-29.130344316551223)--(36,-32.52481468523513)--(37,-37.82149626991834)--(38,-33.733863002400064)--(39,-36.3783907247685)--(40,-32.077107249702834)--(41,-27.472575270636252)--(42,-30.974460084135373)--(43,-37.820907251454464)--(44,-34.169690273585395)--(45,-35.540260020824334)--(46,-37.10860761748474)--(47,-42.98957982398231)--(48,-43.92956903685247)--(49,-37.8301666383021)--(50,-37.124744269771)--(51,-42.068923055506644)--(52,-41.31554196379819)--(53,-43.53141216679537)--(54,-40.81775686118024)--(55,-44.221745390487186)--(56,-50.951255182603404)--(57,-57.40317428155389)--(58,-49.59172634578511)--(59,-49.06038091629415)--(60,-42.298956694572865)--(61,-36.09372615037469)--(62,-28.61499689672624)--(63,-32.53456555232996)--(64,-27.308245636686493)--(65,-34.65050491725552)--(66,-30.849494109166976)--(67,-35.60581505540362)--(68,-39.11855340918012)--(69,-45.53660416910927)--(70,-49.77953806245395)--(71,-53.29538675804117)--(72,-56.1351292497961)--(73,-50.594974837401324)--(74,-53.03290400622324)--(75,-52.6000815734782)--(76,-56.189859518755384)--(77,-50.33903888244133)--(78,-48.99535804307217)--(79,-43.80494898541555)--(80,-46.62146775447714)--(81,-47.40949938001217)--(82,-40.83799525423281)--(83,-39.03458106219348)--(84,-36.75165953402373)--(85,-32.78971111399299)--(86,-30.987110585756515)--(87,-24.06454510946141)--(88,-24.040887963117896)--(89,-25.814828249391304)--(90,-19.421349118681885)--(91,-19.56899411695857)--(92,-22.474718173702136)--(93,-15.938579338612854)--(94,-17.72795628748892)--(95,-16.80687680004351)--(96,-15.120980389207803)--(97,-10.44223514985535)--(98,-4.444882810609173)--(99,0.44377579984027005)--(100,0.35496255098636276)--(101,1.0767271293386758)--(102,-3.3363718920642924)--(103,-1.602232347812512)--(104,2.3667978596305472)--(105,6.85430633927545)--(106,6.887869373573688)--(107,8.211735955349939)--(108,6.726462662519838)--(109,-0.2102666240940323)--(110,-3.083495157299044)--(111,-1.6951118662161857)--(112,-2.899179422511759)--(113,3.135737585729216)--(114,-4.28226532088221)--(115,-11.033986073515596)--(116,-4.146466607540233)--(117,-6.551282420149123)--(118,-11.552357571236536)--(119,-11.642250627744618)--(120,-11.916682961400655)--(121,-14.255048540820205)--(122,-20.69866867740767)--(123,-24.068072079364786)--(124,-22.10513027198744)--(125,-29.85092447410317)--(126,-32.81105050555818)--(127,-36.669076244841854)--(128,-38.68777793504141)--(129,-35.33679118613895)--(130,-42.20889412695256)--(131,-40.415158985517486)--(132,-35.245345710017546)--(133,-28.16869559833743)--(134,-20.817635958992945)--(135,-18.548781923266226)--(136,-12.911049108001952)--(137,-20.471386944232265)--(138,-17.248028903364357)--(139,-23.140780244591447)--(140,-25.27347829101077)--(141,-19.706032586039846)--(142,-18.626532980304674)--(143,-17.313160921571196)--(144,-17.26433861159451)--(145,-16.053646143277682)--(146,-21.416441308604067)--(147,-19.46766266626096)--(148,-18.915147036661303)--(149,-20.77627443039549)--(150,-21.471274509503708)--(151,-19.04139312935944)--(152,-26.557489263926968)--(153,-22.113010540283693)--(154,-22.22218043698998)--(155,-15.440315001540917)--(156,-14.088804576032064)--(157,-18.806757112741103)--(158,-11.366927734149185)--(159,-13.553520078849884)--(160,-13.237350285809788)--(161,-15.988029240730308)--(162,-8.163040809607729)--(163,-13.791645770639553)--(164,-21.907308463387338)--(165,-16.47291056694808)--(166,-14.587963144181966)--(167,-8.058312661348062)--(168,-0.8954942836333828)--(169,-1.2721930869469187)--(170,-16.525585193233887)--(171,-14.17401311090319)--(172,-23.142018654253473)--(173,-17.698727670787573)--(174,-21.485399902562612)--(175,-26.900027778138142)--(176,-19.5757650726945)--(177,-29.57130629899078)--(178,-25.95419339251414)--(179,-30.41272223330651)--(180,-24.762700296397924)--(181,-24.54391848554859)--(182,-25.863313449736065)--(183,-28.182858980523836)--(184,-31.643150641242407)--(185,-32.216704844894)--(186,-26.920366678444594)--(187,-27.273210457752413)--(188,-36.862777847259736)--(189,-26.409458862421175)--(190,-30.674992799923757)--(191,-26.699022753917998)--(192,-32.10794907590446)--(193,-33.43206807249254)--(194,-38.03415492607712)--(195,-35.55016373674483)--(196,-31.84849648604176)--(197,-29.83000646057277)--(198,-38.041709436032484)--(199,-29.687095961210716)--(200,-36.40639258510084);


==> figures/truncation/data_1.tex <==
\draw(0,-0.0)--(200,-40.0);
\draw(0,0.0)--(20,-4.0)--(100,60.0)--(180,-36.0)--(200,-40.0);
\draw(0,12.0)--(20,8.0)--(100,72.0)--(180,-24.0)--(200,-28.0);
\draw(0,24.0)--(20,20.0)--(100,84.0)--(180,-12.0)--(200,-16.0);
\draw(0,-0.0)--(20,-4.0)--(100,-100.0)--(180,-36.0)--(200,-40.0);
\draw(0,-12.0)--(20,-16.0)--(100,-112.0)--(180,-48.0)--(200,-52.0);
\draw(0,-24.0)--(20,-28.0)--(100,-124.0)--(180,-60.0)--(200,-64.0);
\draw(0,0.0)--(1,5.3012295074708735)--(2,6.961260683447953)--(3,6.661200318076056)--(4,-0.8736913672924318)--(5,-4.225192025995522)--(6,-0.6752865723778346)--(7,-4.804844165215168)--(8,-11.382074694779803)--(9,-15.323030889443242)--(10,-18.8921303835474)--(11,-16.252925463491902)--(12,-23.298074322966816)--(13,-26.222504349659076)--(14,-30.275796866798363)--(15,-26.578635505060166)--(16,-23.402591114645)--(17,-28.796803562466067)--(18,-28.331034948516848)--(19,-28.12932202129731)--(20,-35.198006522956156)--(21,-36.62359426073721)--(22,-30.47815784919469)--(23,-34.55602799536713)--(24,-39.9730310680455)--(25,-35.907991229349854)--(26,-41.64089388093422)--(27,-43.60902154475391)--(28,-36.31017235445313)--(29,-30.605765574122596)--(30,-34.60877461391778)--(31,-28.539307746499663)--(32,-33.98007745613776)--(33,-28.16638058426398)--(34,-35.686259414318776)--(35,-29.130344316551223)--(36,-32.52481468523513)--(37,-37.82149626991834)--(38,-33.733863002400064)--(39,-36.3783907247685)--(40,-32.077107249702834)--(41,-27.472575270636252)--(42,-30.974460084135373)--(43,-37.820907251454464)--(44,-34.169690273585395)--(45,-35.540260020824334)--(46,-37.10860761748474)--(47,-42.98957982398231)--(48,-43.92956903685247)--(49,-37.8301666383021)--(50,-37.124744269771)--(51,-42.068923055506644)--(52,-41.31554196379819)--(53,-43.53141216679537)--(54,-40.81775686118024)--(55,-44.221745390487186)--(56,-50.951255182603404)--(57,-57.40317428155389)--(58,-49.59172634578511)--(59,-49.06038091629415)--(60,-42.298956694572865)--(61,-36.09372615037469)--(62,-28.61499689672624)--(63,-32.53456555232996)--(64,-27.308245636686493)--(65,-34.65050491725552)--(66,-30.849494109166976)--(67,-35.60581505540362)--(68,-39.11855340918012)--(69,-45.53660416910927)--(70,-49.77953806245395)--(71,-53.29538675804117)--(72,-56.1351292497961)--(73,-50.594974837401324)--(74,-53.03290400622324)--(75,-52.6000815734782)--(76,-56.189859518755384)--(77,-50.33903888244133)--(78,-48.99535804307217)--(79,-43.80494898541555)--(80,-46.62146775447714)--(81,-47.40949938001217)--(82,-40.83799525423281)--(83,-39.03458106219348)--(84,-36.75165953402373)--(85,-32.78971111399299)--(86,-30.987110585756515)--(87,-24.06454510946141)--(88,-24.040887963117896)--(89,-25.814828249391304)--(90,-19.421349118681885)--(91,-19.56899411695857)--(92,-22.474718173702136)--(93,-15.938579338612854)--(94,-17.72795628748892)--(95,-16.80687680004351)--(96,-15.120980389207803)--(97,-10.44223514985535)--(98,-4.444882810609173)--(99,0.44377579984027005)--(100,0.35496255098636276)--(101,1.0767271293386758)--(102,-3.3363718920642924)--(103,-1.602232347812512)--(104,2.3667978596305472)--(105,6.85430633927545)--(106,6.887869373573688)--(107,8.211735955349939)--(108,6.726462662519838)--(109,-0.2102666240940323)--(110,-3.083495157299044)--(111,-1.6951118662161857)--(112,-2.899179422511759)--(113,3.135737585729216)--(114,-4.28226532088221)--(115,-11.033986073515596)--(116,-4.146466607540233)--(117,-6.551282420149123)--(118,-11.552357571236536)--(119,-11.642250627744618)--(120,-11.916682961400655)--(121,-14.255048540820205)--(122,-20.69866867740767)--(123,-24.068072079364786)--(124,-22.10513027198744)--(125,-29.85092447410317)--(126,-32.81105050555818)--(127,-36.669076244841854)--(128,-38.68777793504141)--(129,-35.33679118613895)--(130,-42.20889412695256)--(131,-40.415158985517486)--(132,-35.245345710017546)--(133,-28.16869559833743)--(134,-20.817635958992945)--(135,-18.548781923266226)--(136,-12.911049108001952)--(137,-20.471386944232265)--(138,-17.248028903364357)--(139,-23.140780244591447)--(140,-25.27347829101077)--(141,-19.706032586039846)--(142,-18.626532980304674)--(143,-17.313160921571196)--(144,-17.26433861159451)--(145,-16.053646143277682)--(146,-21.416441308604067)--(147,-19.46766266626096)--(148,-18.915147036661303)--(149,-20.77627443039549)--(150,-21.471274509503708)--(151,-19.04139312935944)--(152,-26.557489263926968)--(153,-22.113010540283693)--(154,-22.22218043698998)--(155,-15.440315001540917)--(156,-14.088804576032064)--(157,-18.806757112741103)--(158,-11.366927734149185)--(159,-13.553520078849884)--(160,-13.237350285809788)--(161,-15.988029240730308)--(162,-8.163040809607729)--(163,-13.791645770639553)--(164,-21.907308463387338)--(165,-16.47291056694808)--(166,-14.587963144181966)--(167,-8.058312661348062)--(168,-0.8954942836333828)--(169,-1.2721930869469187)--(170,5.966470705709242)--(171,2.313045743030367)--(172,9.381180183938554)--(173,7.636498315517409)--(174,11.082059478371296)--(175,8.026635396244957)--(176,15.798055032167598)--(177,14.400223778222554)--(178,7.7667741380077855)--(179,0.9319224684183176)--(180,4.215600309082275)--(181,1.4690809196942105)--(182,-4.132306431623649)--(183,-4.902286028309119)--(184,-5.219563784795339)--(185,-3.7925737686655197)--(186,-0.243307564562512)--(187,-4.048647962053458)--(188,-5.157147251193392)--(189,-0.4036927064694211)--(190,-1.8706418844847406)--(191,-5.192934855606662)--(192,0.06482332612696595)--(193,-6.538328529239919)--(194,-12.737667963746931)--(195,-13.185173587585998)--(196,-9.047880749495741)--(197,-5.587754402208647)--(198,-2.910009484736488)--(199,-4.309803545910075)--(200,0.0);
\draw(0,0.0)--(1,5.3012295074708735)--(2,6.961260683447953)--(3,6.661200318076056)--(4,-0.8736913672924318)--(5,-4.225192025995522)--(6,-0.6752865723778346)--(7,-4.804844165215168)--(8,-11.382074694779803)--(9,-15.323030889443242)--(10,-18.8921303835474)--(11,-16.252925463491902)--(12,-23.298074322966816)--(13,-26.222504349659076)--(14,-30.275796866798363)--(15,-26.578635505060166)--(16,-23.402591114645)--(17,-28.796803562466067)--(18,-28.331034948516848)--(19,-28.12932202129731)--(20,-35.198006522956156)--(21,-36.62359426073721)--(22,-30.47815784919469)--(23,-34.55602799536713)--(24,-39.9730310680455)--(25,-35.907991229349854)--(26,-41.64089388093422)--(27,-43.60902154475391)--(28,-36.31017235445313)--(29,-30.605765574122596)--(30,-34.60877461391778)--(31,-28.539307746499663)--(32,-33.98007745613776)--(33,-28.16638058426398)--(34,-35.686259414318776)--(35,-29.130344316551223)--(36,-32.52481468523513)--(37,-37.82149626991834)--(38,-33.733863002400064)--(39,-36.3783907247685)--(40,-32.077107249702834)--(41,-27.472575270636252)--(42,-30.974460084135373)--(43,-37.820907251454464)--(44,-34.169690273585395)--(45,-35.540260020824334)--(46,-37.10860761748474)--(47,-42.98957982398231)--(48,-43.92956903685247)--(49,-37.8301666383021)--(50,-37.124744269771)--(51,-42.068923055506644)--(52,-41.31554196379819)--(53,-43.53141216679537)--(54,-40.81775686118024)--(55,-44.221745390487186)--(56,-50.951255182603404)--(57,-57.40317428155389)--(58,-49.59172634578511)--(59,-49.06038091629415)--(60,-42.298956694572865)--(61,-36.09372615037469)--(62,-28.61499689672624)--(63,-32.53456555232996)--(64,-27.308245636686493)--(65,-34.65050491725552)--(66,-30.849494109166976)--(67,-35.60581505540362)--(68,-39.11855340918012)--(69,-45.53660416910927)--(70,-49.77953806245395)--(71,-53.29538675804117)--(72,-56.1351292497961)--(73,-50.594974837401324)--(74,-53.03290400622324)--(75,-52.6000815734782)--(76,-56.189859518755384)--(77,-50.33903888244133)--(78,-48.99535804307217)--(79,-43.80494898541555)--(80,-46.62146775447714)--(81,-47.40949938001217)--(82,-40.83799525423281)--(83,-39.03458106219348)--(84,-36.75165953402373)--(85,-32.78971111399299)--(86,-30.987110585756515)--(87,-24.06454510946141)--(88,-24.040887963117896)--(89,-25.814828249391304)--(90,-19.421349118681885)--(91,-19.56899411695857)--(92,-22.474718173702136)--(93,-15.938579338612854)--(94,-17.72795628748892)--(95,-16.80687680004351)--(96,-15.120980389207803)--(97,-10.44223514985535)--(98,-4.444882810609173)--(99,0.44377579984027005)--(100,0.35496255098636276)--(101,1.0767271293386758)--(102,-3.3363718920642924)--(103,-1.602232347812512)--(104,2.3667978596305472)--(105,6.85430633927545)--(106,6.887869373573688)--(107,8.211735955349939)--(108,6.726462662519838)--(109,-0.2102666240940323)--(110,-3.083495157299044)--(111,-1.6951118662161857)--(112,-2.899179422511759)--(113,3.135737585729216)--(114,-4.28226532088221)--(115,-11.033986073515596)--(116,-4.146466607540233)--(117,-6.551282420149123)--(118,-11.552357571236536)--(119,-11.642250627744618)--(120,-11.916682961400655)--(121,-14.255048540820205)--(122,-20.69866867740767)--(123,-24.068072079364786)--(124,-22.10513027198744)--(125,-29.85092447410317)--(126,-32.81105050555818)--(127,-36.669076244841854)--(128,-38.68777793504141)--(129,-35.33679118613895)--(130,-42.20889412695256)--(131,-40.415158985517486)--(132,-35.245345710017546)--(133,-28.16869559833743)--(134,-20.817635958992945)--(135,-18.548781923266226)--(136,-12.911049108001952)--(137,-20.471386944232265)--(138,-17.248028903364357)--(139,-23.140780244591447)--(140,-25.27347829101077)--(141,-19.706032586039846)--(142,-18.626532980304674)--(143,-17.313160921571196)--(144,-17.26433861159451)--(145,-16.053646143277682)--(146,-21.416441308604067)--(147,-19.46766266626096)--(148,-18.915147036661303)--(149,-20.77627443039549)--(150,-21.471274509503708)--(151,-19.04139312935944)--(152,-26.557489263926968)--(153,-22.113010540283693)--(154,-22.22218043698998)--(155,-15.440315001540917)--(156,-14.088804576032064)--(157,-18.806757112741103)--(158,-11.366927734149185)--(159,-13.553520078849884)--(160,-13.237350285809788)--(161,-15.988029240730308)--(162,-8.163040809607729)--(163,-13.791645770639553)--(164,-21.907308463387338)--(165,-16.47291056694808)--(166,-14.587963144181966)--(167,-8.058312661348062)--(168,-0.8954942836333828)--(169,-1.2721930869469187)--(170,-16.525585193233887)--(171,-14.17401311090319)--(172,-23.142018654253473)--(173,-17.698727670787573)--(174,-21.485399902562612)--(175,-26.900027778138142)--(176,-19.5757650726945)--(177,-29.57130629899078)--(178,-25.95419339251414)--(179,-30.41272223330651)--(180,-24.762700296397924)--(181,-24.54391848554859)--(182,-25.863313449736065)--(183,-28.182858980523836)--(184,-31.643150641242407)--(185,-32.216704844894)--(186,-26.920366678444594)--(187,-27.273210457752413)--(188,-36.862777847259736)--(189,-26.409458862421175)--(190,-30.674992799923757)--(191,-26.699022753917998)--(192,-32.10794907590446)--(193,-33.43206807249254)--(194,-38.03415492607712)--(195,-35.55016373674483)--(196,-31.84849648604176)--(197,-29.83000646057277)--(198,-38.041709436032484)--(199,-29.687095961210716)--(200,-36.40639258510084);
\draw(0,0.0)--(1,5.3012295074708735)--(2,6.961260683447953)--(3,6.661200318076056)--(4,-0.8736913672924318)--(5,-4.225192025995522)--(6,-0.6752865723778346)--(7,-4.804844165215168)--(8,-11.382074694779803)--(9,-15.323030889443242)--(10,-18.8921303835474)--(11,-16.252925463491902)--(12,-23.298074322966816)--(13,-26.222504349659076)--(14,-4.702007941022742)--(15,-26.578635505060166)--(16,-23.402591114645)--(17,-15.005497204858944)--(18,-8.335852633615719)--(19,-11.909722571725101)--(20,-10.354532723354126)--(21,-6.040889496730662)--(22,-7.792086830399798)--(23,-12.80272945906366)--(24,-13.204811350196728)--(25,-18.544516205832)--(26,-16.900732490133663)--(27,-23.945797335412536)--(28,-36.31017235445313)--(29,-30.605765574122596)--(30,-34.60877461391778)--(31,-28.539307746499663)--(32,-33.98007745613776)--(33,-28.16638058426398)--(34,-35.686259414318776)--(35,-29.130344316551223)--(36,-32.52481468523513)--(37,-37.82149626991834)--(38,-33.733863002400064)--(39,-36.3783907247685)--(40,-32.077107249702834)--(41,-27.472575270636252)--(42,-30.974460084135373)--(43,-37.820907251454464)--(44,-34.169690273585395)--(45,-35.540260020824334)--(46,-37.10860761748474)--(47,-42.98957982398231)--(48,-43.92956903685247)--(49,-37.8301666383021)--(50,-37.124744269771)--(51,-42.068923055506644)--(52,-41.31554196379819)--(53,-43.53141216679537)--(54,-40.81775686118024)--(55,-44.221745390487186)--(56,-50.951255182603404)--(57,-57.40317428155389)--(58,-49.59172634578511)--(59,-49.06038091629415)--(60,-42.298956694572865)--(61,-36.09372615037469)--(62,-28.61499689672624)--(63,-32.53456555232996)--(64,-27.308245636686493)--(65,-34.65050491725552)--(66,-30.849494109166976)--(67,-35.60581505540362)--(68,-39.11855340918012)--(69,-45.53660416910927)--(70,-49.77953806245395)--(71,-53.29538675804117)--(72,-56.1351292497961)--(73,-50.594974837401324)--(74,-53.03290400622324)--(75,-52.6000815734782)--(76,-56.189859518755384)--(77,-50.33903888244133)--(78,-48.99535804307217)--(79,-43.80494898541555)--(80,-46.62146775447714)--(81,-47.40949938001217)--(82,-40.83799525423281)--(83,-39.03458106219348)--(84,-36.75165953402373)--(85,-32.78971111399299)--(86,-30.987110585756515)--(87,-24.06454510946141)--(88,-24.040887963117896)--(89,-25.814828249391304)--(90,-19.421349118681885)--(91,-19.56899411695857)--(92,-22.474718173702136)--(93,-15.938579338612854)--(94,-17.72795628748892)--(95,-16.80687680004351)--(96,-15.120980389207803)--(97,-10.44223514985535)--(98,-4.444882810609173)--(99,0.44377579984027005)--(100,0.35496255098636276)--(101,1.0767271293386758)--(102,-3.3363718920642924)--(103,-1.602232347812512)--(104,2.3667978596305472)--(105,6.85430633927545)--(106,6.887869373573688)--(107,8.211735955349939)--(108,6.726462662519838)--(109,-0.2102666240940323)--(110,-3.083495157299044)--(111,-1.6951118662161857)--(112,-2.899179422511759)--(113,3.135737585729216)--(114,-4.28226532088221)--(115,-11.033986073515596)--(116,-4.146466607540233)--(117,-6.551282420149123)--(118,-11.552357571236536)--(119,-11.642250627744618)--(120,-11.916682961400655)--(121,-14.255048540820205)--(122,-20.69866867740767)--(123,-24.068072079364786)--(124,-22.10513027198744)--(125,-29.85092447410317)--(126,-32.81105050555818)--(127,-36.669076244841854)--(128,-38.68777793504141)--(129,-35.33679118613895)--(130,-42.20889412695256)--(131,-40.415158985517486)--(132,-35.245345710017546)--(133,-28.16869559833743)--(134,-20.817635958992945)--(135,-18.548781923266226)--(136,-12.911049108001952)--(137,-20.471386944232265)--(138,-17.248028903364357)--(139,-23.140780244591447)--(140,-25.27347829101077)--(141,-19.706032586039846)--(142,-18.626532980304674)--(143,-17.313160921571196)--(144,-17.26433861159451)--(145,-16.053646143277682)--(146,-21.416441308604067)--(147,-19.46766266626096)--(148,-18.915147036661303)--(149,-20.77627443039549)--(150,-21.471274509503708)--(151,-19.04139312935944)--(152,-26.557489263926968)--(153,-22.113010540283693)--(154,-22.22218043698998)--(155,-15.440315001540917)--(156,-14.088804576032064)--(157,-18.806757112741103)--(158,-11.366927734149185)--(159,-13.553520078849884)--(160,-13.237350285809788)--(161,-15.988029240730308)--(162,-8.163040809607729)--(163,-13.791645770639553)--(164,-21.907308463387338)--(165,-16.47291056694808)--(166,-14.587963144181966)--(167,-8.058312661348062)--(168,-0.8954942836333828)--(169,-1.2721930869469187)--(170,-16.525585193233887)--(171,-14.17401311090319)--(172,-23.142018654253473)--(173,-17.698727670787573)--(174,-21.485399902562612)--(175,-26.900027778138142)--(176,-19.5757650726945)--(177,-29.57130629899078)--(178,-25.95419339251414)--(179,-30.41272223330651)--(180,-24.762700296397924)--(181,-24.54391848554859)--(182,-25.863313449736065)--(183,-28.182858980523836)--(184,-31.643150641242407)--(185,-32.216704844894)--(186,-26.920366678444594)--(187,-27.273210457752413)--(188,-36.862777847259736)--(189,-26.409458862421175)--(190,-30.674992799923757)--(191,-26.699022753917998)--(192,-32.10794907590446)--(193,-33.43206807249254)--(194,-38.03415492607712)--(195,-35.55016373674483)--(196,-31.84849648604176)--(197,-29.83000646057277)--(198,-38.041709436032484)--(199,-29.687095961210716)--(200,-36.40639258510084);


==> sections/middle/07_limit_equalities_03_ergodic_approx_fig_wash.tex <==
%!TEX root=../../main.tex

\begin{figure}

  \newcommand{\sband}[3]{
    \fill[color=black!#3]
      (#1,   10   )--
      (#2, 10   )--
      (#2-5,0)--
      (#1-5,0)--
      cycle;
  }
  \newcommand{\rect}[2]{
    \draw (#1 * 0.7-0.2,#2 * 0.7-0.2) rectangle (#1 * 0.7+0.3,#2 * 0.7+0.3);
  }

\begin{center}
  \begin{subfigure}[t]{0.4\textwidth}
    \centering
    \begin{tikzpicture}[x=0.6cm, y=0.6cm]
      \begin{scope}
        \clip (-0.1,-0.1) rectangle (10.1,10.1);
        \begin{scope}
          \clip (0,0) rectangle (10,10);
          \sband{0}{2}{10}
          \sband{2}{4}{30}
          \sband{4}{6}{10}
          \sband{6}{8}{30}
          \sband{8}{10}{10}
          \sband{10}{12}{30}
          \sband{12}{14}{10}
          \sband{14}{16}{30}
        \end{scope}

        \node at (2,8.5)[anchor=north] {$u_\mu$};
        \node at (4,8.5)[anchor=north] {$u_\nu$};

      \end{scope}
    \end{tikzpicture}
    \caption{The gradient of $f$}
    \label{figure_washboard_new_gradient}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.4\textwidth}
    \centering
    \begin{tikzpicture}[x=0.6cm, y=0.6cm]
      \begin{scope}
        \clip (-0.1,-0.1) rectangle (11.3,10.1);
        \fill[color=black] (0,0)rectangle(10,10);
        \fill[color=white] (0.05,0.05)rectangle(9.95,9.95);
        \begin{scope}
          \clip (1,1) rectangle (9,9);
          \sband{0}{2}{10}
          \sband{2}{4}{30}
          \sband{4}{6}{10}
          \sband{6}{8}{30}
          \sband{8}{10}{10}
          \sband{10}{12}{30}
          \sband{12}{14}{10}
          \sband{14}{16}{30}
        \end{scope}

                % \rect{2}{2}
                \rect{2}{3}
                \rect{2}{4}
                \rect{2}{5}
                % \rect{2}{6}
                % \rect{2}{7}
                % \rect{2}{8}
                \rect{2}{9}
                \rect{2}{10}
                \rect{2}{11}
                % \rect{2}{12}

                        %
                        % \rect{3}{2}
                        % \rect{3}{3}
                        % \rect{3}{4}
                        \rect{3}{5}
                        \rect{3}{6}
                        \rect{3}{7}
                        % \rect{3}{8}
                        % \rect{3}{9}
                        % \rect{3}{10}
                        \rect{3}{11}
                        \rect{3}{12}

                        \rect{4}{2}
                        \rect{4}{3}
                        % \rect{4}{4}
                        % \rect{4}{5}
                        % \rect{4}{6}
                        \rect{4}{7}
                        \rect{4}{8}
                        \rect{4}{9}
                        % \rect{4}{10}
                        % \rect{4}{11}
                        % \rect{4}{12}

                        % \rect{5}{2}
                        \rect{5}{3}
                        \rect{5}{4}
                        \rect{5}{5}
                        % \rect{5}{6}
                        % \rect{5}{7}
                        % \rect{5}{8}
                        \rect{5}{9}
                        \rect{5}{10}
                        \rect{5}{11}
                        % \rect{5}{12}

                        \rect{6}{2}
                        % \rect{6}{3}
                        % \rect{6}{4}
                        \rect{6}{5}
                        \rect{6}{6}
                        \rect{6}{7}
                        % \rect{6}{8}
                        % \rect{6}{9}
                        % \rect{6}{10}
                        \rect{6}{11}
                        \rect{6}{12}

                        \rect{7}{2}
                        \rect{7}{3}
                        \rect{7}{4}
                        % \rect{7}{5}
                        % \rect{7}{6}
                        \rect{7}{7}
                        \rect{7}{8}
                        \rect{7}{9}
                        % \rect{7}{10}
                        % \rect{7}{11}
                        % \rect{7}{12}

                        % \rect{8}{2}
                        % \rect{8}{3}
                        \rect{8}{4}
                        \rect{8}{5}
                        \rect{8}{6}
                        % \rect{8}{7}
                        % \rect{8}{8}
                        \rect{8}{9}
                        \rect{8}{10}
                        \rect{8}{11}
                        % \rect{8}{12}

                        \rect{9}{2}
                        % \rect{9}{3}
                        % \rect{9}{4}
                        % \rect{9}{5}
                        \rect{9}{6}
                        \rect{9}{7}
                        \rect{9}{8}
                        % \rect{9}{9}
                        % \rect{9}{10}
                        \rect{9}{11}
                        \rect{9}{12}                        \rect{10}{2}
                          \rect{10}{3}
                          \rect{10}{4}
                          % \rect{10}{5}
                          % \rect{10}{6}
                          % \rect{10}{7}
                          \rect{10}{8}
                          \rect{10}{9}
                          \rect{10}{10}
                          % \rect{10}{11}
                          % \rect{10}{12}

                          % \rect{11}{2}
                          % \rect{11}{3}
                          \rect{11}{4}
                          \rect{11}{5}
                          \rect{11}{6}
                          % \rect{11}{7}
                          % \rect{11}{8}
                          % \rect{11}{9}
                          \rect{11}{10}
                          \rect{11}{11}
                          \rect{11}{12}
                          \rect{12}{2}
                          % \rect{12}{3}
                          % \rect{12}{4}
                          % \rect{12}{5}
                          \rect{12}{6}
                          \rect{12}{7}
                          \rect{12}{8}
                          % \rect{12}{9}
                          % \rect{12}{10}
                          % \rect{12}{11}
                          \rect{12}{12}


\draw[decorate,decoration={brace,amplitude=0.1cm}](10.1,10)--(10.1,0);
\node at (10.2,5.15) [anchor=west] {$n^5$};
\draw[decorate,decoration={brace,amplitude=0.1cm}](10.3,10)--(10.3,9);
\node at (10.4,9.65) [anchor=west] {$n^4$};
\draw[decorate,decoration={brace,amplitude=0.1cm}](1.5,9.1)--(3.5,9.1);
\node at (2.65,9.15) [anchor=south] {$n^3$};
\draw [decorate,decoration={brace,amplitude=0.05cm}](8.8,5.9)--(8.8,5.4);
\node at (8.8,5.8) [anchor=west] {$n^2$};
\draw [decorate,decoration={brace,amplitude=0.025cm}](8.8,4.7)--(8.8,4.5);
\node at (8.8,4.6) [anchor=west] {$n$};


\end{scope}



    \end{tikzpicture}
    \caption{Overview of the construction}
    \label{figure_washboard_new_sets}
  \end{subfigure}
  \caption{The washboard}
  \label{figure_washboard}
\end{center}
\end{figure}


==> sections/middle/10_LDP_03_corollary.tex <==
%!TEX root=../../main.tex


\color{blue}
\textbf{Let's focus on this later, we should use monotonicity somewhere too here and
there should be a short argument}

Before proving Theorem~\ref{p_LDP}, let us also state a direct corollary obtained by restricting the LDP to the second coordinate of $M^*(D\times\Omega) \times\operatorname{Lip}_K(\bar D)$. This corollary is the analogous for monotone Lipschitz random surfaces of the variational principle proved in~\cite{CKP01} for domino tilings.
%For $(D_n, \psi^n)_{n\in \mathbb N}$ denote a good approximation of the good
%asymptotic profile $(D,f)$. define a measure $\kappa_n$ induced by sampling  a configuration $\psi^n$ from $\gamma_{D_n}(\cdot,\phi^n)$ and applying the map $\mathfrak G_n(\phi)$ to $\psi^n$.
\begin{corollary}
	[Variational principle for the macroscopic limit]\label{p_VP}
 Let $(D_n, \psi^n)_{n\in \mathbb N}$ denote a good approximation of the good
asymptotic profile $(D,f)$. For all $n$, define by $\kappa_n$ the measure induced by sampling  a configuration $\psi^n$ from $\gamma_{D_n}(\cdot,\phi^n)$ and applying the map $\mathfrak G_n$ to $\psi^n$.
The sequence $(\kappa_n)_{n \in N}$ satisfy a large deviation principle with speed $n^d$ and rate function
	\[
	I(f) := \begin{cases}
	\int_D \sigma(\nabla f)dx - P_{\Phi}(D,g)
	&\text{if $f|_{\partial R} = g$} \,, \\
	\infty
	&\text{otherwise} \,.
	\end{cases}
	\]
	on the space $\operatorname{Lip}_K(\bar D)$ in the topology  $\mathcal X^\infty$.
\end{corollary}


\color{black}

